Adversarial robustness via robust low rank representations

Adversarial robustness measures the susceptibility of a classifier to imperceptible perturbations made to the inputs at test time. In this work we highlight the benefits of natural low rank representations that often exist for real data such as images, for training neural networks with certified robustness guarantees. Our first contribution is for certified robustness to perturbations measured in $\ell_2$ norm. We exploit low rank data representations to provide improved guarantees over state-of-the-art randomized smoothing-based approaches on standard benchmark datasets such as CIFAR-10 and CIFAR-100. Our second contribution is for the more challenging setting of certified robustness to perturbations measured in $\ell_\infty$ norm. We demonstrate empirically that natural low rank representations have inherent robustness properties, that can be leveraged to provide significantly better guarantees for certified robustness to $\ell_\infty$ perturbations in those representations. Our certificate of $\ell_\infty$ robustness relies on a natural quantity involving the $\infty \to 2$ matrix operator norm associated with the representation, to translate robustness guarantees from $\ell_2$ to $\ell_\infty$ perturbations. A key technical ingredient for our certification guarantees is a fast algorithm with provable guarantees based on the multiplicative weights update method to provide upper bounds on the above matrix norm. Our algorithmic guarantees improve upon the state of the art for this problem, and may be of independent interest.

==> oldmwanalysis.tex <==
% !TEX root = main.tex


\subsection{Certifying the $\infty \to 2$ operator norm} \label{sec:mw}

We now describe our efficient algorithmic procedure that gives a certifies an upper bound on the $\infty \to 2$ norm of the given matrix. Moreover, as we will see in Theorem~\ref{thm:optimal-guarantee-sdp}, our algorithmic procedure comes with provable guarantees: it is guaranteed to output a value that is only a small constant factor off from the global optimum i.e., true value of the $\infty \to 2$ norm. 

We first note that $\| A\|_{\infty \to 2}^2 = \|A^\top A\|_{\infty \to 1}$.  Moreover, by the variational characterization of operator norms, we have for $M=A A^\top \succeq 0$
\begin{equation} \label{eq:operator:problem}
\|A\|_{\infty \to 2}^2 = \max_{x: \|{x}\|_\infty \le 1}\max_{y: \|{y}\|_\infty \le 1} x^\top M y = \max_{x: \|{x}\|_\infty \le 1}x^\top M x.
\end{equation}

We consider the following standard SDP relaxation for the problem \eqref{eq:primal}, where $M \succeq 0$. The primal variables are represented by the positive semi-definite (PSD) matrix $X \in \R^{n \times n}$. The SDP dual of this relaxation, given in \eqref{eq:dual}l, has variables $y_1, \dots, y_n \ge 0$ corresponding to the $n$ constraints \eqref{eq:primal:const1}. In what follows, for matrices $M,X$, $\iprod{M,X}:=\tr(M^\top X)$ represents the trace inner product. 

\fboxsep=0pt
\noindent\fbox{%
\vspace{5pt}
\noindent\begin{minipage}{.48\linewidth}
%{\bf Primal:}
\begin{align}\label{eq:primal}
{\textbf{Primal SDP:}}~~~
\max_{X} & ~ \iprod{M,X} \\
\text{ s.t. } ~~~& X_{ii} \le 1, ~~~\forall i \in [n] \label{eq:primal:const1}\\
& X \succeq 0. \nonumber
\end{align}
\end{minipage}%
~~~\vline~~~
\begin{minipage}{.48\linewidth}
%{\bf Dual:}
\begin{align}\label{eq:dual}
\textbf{Dual SDP:}~~~ 
\min_{y} & ~ \sum_{i \in [n]} y_i \\
\text{ s.t. } ~~~& diag(y) \succeq M  \label{eq:dual:const2}\\
& y \ge 0. \nonumber
\end{align}
\end{minipage}
~

\vspace{3pt}
}

Recall that our algorithm goal is to output a value that is guaranteed to be a valid upper bound for $\norm{A}_{\infty \to 2}^2 = \norm{M}_{\infty \to 1}$.\footnote{Hence a fast algorithm that potentially finds a local optimum for the problem will not suffice for our purposes; we need an upper bound on the global optimum of \eqref{eq:operator:problem}.}  
The above primal SDP~\eqref{eq:primal} is a valid relaxation; hence it gives an upper bound on the $\norm{M}_{\infty \to 1}$. % operator norm of $M$. 
Moreover by weak duality, any feasible solution to the dual SDP~\eqref{eq:dual} gives a valid upper bound for the primal SDP value, and hence $\norm{M}_{\infty \to 1}$. However, the above SDP is computationally intensive to solve using off-the-shelf SDP solvers (even for CIFAR-10 images, $X$ is $1024 \times 1024$) \anote{Justify this better.}. Instead we use an algorithmic from the {\em multiplicative weight update} (MWU) framework for solving convex relaxations ~\cite{PlotkinShmoys,KleinLu,AroraHazanKale}. 

\paragraph{Description of the algorithm}

\newcommand{\cub}{\text{val}_{\text{curr}}}
\newcommand{\valub}{\text{val}_{\text{ub}}}
\newcommand{\cuy}{\text{y}_{\text{curr}}}
\newcommand{\miny}{y_{\text{best}}}
\newcommand{\minval}{\text{dobj}_{\text{best}}}

Our algorithm slightly differs from the standard MWU approach for solving the above SDP. The following algorithm takes in as input a PSD matrix $M$ and always returns an upper bound $\valub$ on the SDP value, along with a dual certificate (a dual feasible solution $y$ that attains a dual objective value of $\valub$), and candidate primal solution $X$ that attains the same value (and is potentially feasible). Theorem~\ref{thm:sdp-guarantee} proves that for the right setting of parameters, particularly $T_f = O(n \log n/ \eps^2)$, the solution $X$ is also guaranteed to be feasible up to small error $\eta>0$.    




\begin{algorithm}[H]
\caption{Fast Certification of $\infty \to 1$ norm}
\label{algo:sdp}
\begin{algorithmic}[1]
\Function{CertifySDP}{PSD matrix $M \in \R^{n \times n}$, iteration bound $T_f$, slack $\eps$, damping $\rho$}
\State Set $T=\min\set{O(n \log n / \eps^2), T_f}$.
\State Initialize $\alpha=(1,1,\dots,1) \in \R^n$. $X=I, y=0^n$, $\minval=\infty$, $\miny=0^n$.
\For{$t=0,1 \dots,  T$} 
    \State $\lambda \gets \text{max-eigenvalue}(\diag(\alpha)^{-1/2} M \diag(\alpha)^{-1/2})$ and $u \in \R^n$ be its eigenvector. 
    \State $v \gets \sqrt{n} \cdot \diag(\alpha)^{-1/2} u $ and $\cub = n \lambda$, $\cuy=\lambda \alpha$.
    \State $y \gets \tfrac{1}{t+1} (t y + \cuy)$, $X \gets \tfrac{1}{t+1}(t X + vv^\top)$. \label{eq:iterate:def}
  %  \State Check conditions for \textit{Early Stop} and return output as appropriate. 
     \If {$\norm{v}_\infty \le 1+\eps$} 
         \State Do early stop and return $\cub$ and $\cuy$, $X=v v^\top$.
   %  \ElsIf{$\max_i |X_{ii}| \le 1+\eta$}
   %         \State Do early stop and return $val_{ub}=\sum_{i=1}^n y_i$, $y$ and $X$.  
     \EndIf
    \State Update weights $\alpha \gets \text{UpdateWeights}(\alpha,v,\rho)$.   
%    \State For each $i \in [n]$, update $\alpha(i) \gets \alpha(i) \exp\big(-\tfrac{\eps}{\rho}(v(i)^2 -1)\big)$. 
%    \State Renormalize $\alpha$ so that $\sum_{i=1}^n \alpha(i)=n$.
    \State {\bf if} $\cub < \minval$, {\bf then} set $\minval=\cub$ and $\miny=y$.
%    \State $t \gets t+1$.  
\EndFor   
\State Output $\minval$, dual solution $\miny$ (certificate), and primal candidate $\widehat{X}$. 

%\For{$i=1,2,\cdots,t$}
%\If{$|P|=1$}
%\State return P
%\EndIf
%\EndFor
\EndFunction
\end{algorithmic}
\end{algorithm}
\anote{We need to reword this algorithm to make it more effective. Maybe state the early stopping conditions separately?}

In the above algorithm, there are weights given by $\alpha$ for $n$ different constraints of the form $X_{ii} \le 1$ \eqref{eq:primal:const1}. At each iteration, the algorithm maximizes the objective subject to {\em one} constraint of the form $\sum_i \alpha_i X_{ii} \le n$. This is done using a maximum eigenvalue/eigenvector computation. We use the following simple multiplicative weight update to update the weights $\alpha$, based on the violation of the solution found in the current iterate.  

\begin{algorithm}[H]
\caption{Update Weights}
\label{algo:weightupdate}
\begin{algorithmic}[1]
\Function{Update Weights}{weights $\alpha \in \R^{n}$, vector $v$, damping $\rho$}

    \State For each $i \in [n]$, update $\alpha(i) \gets \alpha(i) \exp\big(\frac{1}{\rho}(v(i)^2 -1)\big)$. 
    \State Renormalize $\alpha$ so that $\sum_{i=1}^n \alpha(i)=n$. Output $\alpha$. 
% \State For each $j \in [m]$, let $A'_j = \tfrac{1}{\sqrt{2}}(\tilde{A}_j - \tilde{A}_{m+j})$ and let $A''_j = \tfrac{1}{\sqrt{2}}(\tilde{A}_{2m+j} - \tilde{A}_{3m+j})$. \label{st:sym}
% \State Run \textsc{RobustProjection}$(A', r, \kappa,q)$ to find a $r$-dimensional projection matrix $\widehat{\Pi}$. 
\EndFunction
\end{algorithmic}
\end{algorithm}

Our algorithm differs from the standard MWU approach (and analysis)~\cite{Kalethesis} treats the constraints \eqref{eq:primal:const1} and the objective~\eqref{eq:primal} similarly. Firstly, we always maintain a dual feasible solution that gives a valid upper bound on the objective value -- this allows us to do an early stop if appropriate. Secondly, by treating the objective differently from the constraints, we ensure that the width of the convex program is smaller; this allows us to get a better convergence guarantee. 

The damping factors $\rho$ determines the rate of progress of the iterations -- the smaller the value of $\rho$, the faster the progress. The theoretical guarantees for Theorem~\ref{thm:sdp-guarantee} choose $\rho=\Omega(n)$ to avoid any potential oscillating behavior, and provably solve the SDP to optimality. A more aggressive (smaller) choice of seems to work well in practice, in giving faster convergence guarantees (see \ref{sec:sdp:experiments}). Finally, we remark that for {\em every} choice of $\alpha$ (and the update rule), $\cub=n\lambda$ gives a valid upper bound (due to dual feasibility). This is encapsulated in the following simple proposition %. Here for any symmetric matrix $B$, $\lambda_{\max}(B)$ refers to the maximum eigenvalue of matrix $B$, and
where $\text{sdpval}$ refers to the optimal solution value of the \eqref{eq:primal}.    

\begin{proposition} \label{prop:}
For any $\alpha \in \R_{\ge 0}^n $ with $\sum_{i=1}^n \alpha(i) =n$, if $\lambda$ is the maximum eigenvalue %of $(\diag(\alpha)^{-1/2} M \diag(\alpha)^{-1/2})$, then 
%(i) $\text{sdpval} \le n \lambda$,
%$\lambda_{\max}(\cdot)$ the maximum eigenvalue then 
$$\lambda = \lambda_{\max}\Big( (\diag(\alpha)^{-1/2} M \diag(\alpha)^{-1/2}) \Big), \text{ then we have} \text{sdpval} \le n \lambda,$$
and $y=\lambda \alpha$ is feasible for the dual SDP \eqref{eq:dual} and attains an objective value of $n \lambda$. 
\end{proposition}
\begin{proof}
Consider $y= \lambda \alpha$. Firstly, the dual objective value at $y$ is $\sum_{i=1}^n y_i = \lambda \sum_i \alpha(i) = n\lambda$, as required. Moreover $y \ge 0$, since the $\alpha \ge 0$. Finally, \eqref{eq:dual:const2} is satisfied since by definition of $\lambda$, 
\begin{align*}
    \diag(\alpha)^{-1/2} M \diag(\alpha)^{-1/2} \preceq \lambda \cdot I ~~\implies~~ M \preceq \lambda \cdot \diag(\alpha) = \diag(y),  
\end{align*}
by pre-multiplying and post-multiplying by $\diag(\alpha)^{1/2}$. Finally, from weak duality $\text{sdpval} \le n \lambda$. 
\end{proof}

\paragraph{Early Stopping and Other Heuristics. }
There are several conditions for valid {\em early stopping } that can significantly speed up the algorithm. We list some of them below. 
\begin{itemize}
    \item  
    \item 
\end{itemize}


\paragraph{Analysis of the algorithm}

We show the following guarantee for our algorithm. 

\begin{theorem}\label{thm:sdp-guarantee}
For any $\eps>0$, PSD matrix $M$, Algorithm~\ref{algo:sdp} on input $M$, with parameters $\eps$ and $\rho=O(n)$ after $T=O(n \log n/\eps^2)$ iterations finds a solution $\widehat{X} \in \R^{n \times n}$ and $\widehat{y} \in \R^n$ such that 

\vspace{-\topsep}
\begin{enumerate}
\setlength{\parskip}{0pt}
  \setlength{\itemsep}{0pt plus 1pt}
    \item[(a)] $\widehat{y}$ is feasible for the dual SDP \eqref{eq:dual} such that $\iprod{M,\widehat{X}} = \sum_{i=1}^n y_i$.  
    \item[(b)] $\widehat{X} \succeq 0$, $\widehat{X}_{ii} \le 1+\eps$ for all $i \in [n]$, and $\iprod{M, \widehat{X}}=\text{sdpval}$, the primal SDP value.
\end{enumerate}
\vspace{-\topsep}
\end{theorem}
The analysis closely mirrors the analysis of the Multiplicative Weights algorithm for solving SDPs due to Klein and Lu~\cite{KleinLu}, and Arora, Hazan and Kale (see \cite{AroraHK,Kalethesis}). The main parameter that affects the running time of the multiplicative weights update method is the width parameter $\rho'$ of the SDP constraints. The analysis of Klein and Lu ~\cite{KleinLu} is specialized for the Max-Cut problem (which is a special case of \eqref{eq:operator:problem} where $M$ is a graph Laplacian), where they achieve a similar bound of $O(n\log n/\eps^2)$ eigenvalue computations; however their analysis does not directly extend to our more general setting.  In the general framework of \cite{AroraHK}, the optimization problem is first converted into a feasibility problem (hence the objective also becomes a constraint). For SDPs of the form \eqref{eq:primal}, the width parameter could be reasonably large and could result in $\omega(n^3)$ iterations (see Section 6.3 of \cite{Kalethesis}). In our analysis, we ensure that the width is small by treating the objective separately from the constraints. Finally, we present a slightly different analysis using the SDP dual, that has the additional benefit of providing a certificate of optimality. 
\anote{Mention explicit improvement over Kale thesis for QP? Does our result apply to general QP?}

\paragraph{Proof of Theorem~\ref{thm:sdp-guarantee}.}
%We establish the Theorem in the case when $M$ is PSD (this is the situation for our desired problem ~\eqref{eq:operator:problem}. But the same analysis also applies in a more general setting of the Quadratic Programming problem (QP). 

Let at step $t$ of the iteration, $\alpha^{(t)}$ be the weight vector, $X^{(t)}$ be the candidate SDP solution and  $y^{(t)}$ be the candidate dual solution maintained by the Algorithm~\ref{algo:sdp} in step \ref{eq:iterate:def}. It is easy to see that
\begin{align*}
  \forall t \le T,~~  X^{(t)} &= \frac{1}{t}\sum_{\ell=1}^t v^{(\ell)} (v^{(\ell)})^\top, ~~~ \text{and  }~\quad~  y^{(t)} = \frac{1}{t}\sum_{\ell=1}^t \lambda^{(\ell)} \alpha^{(\ell)}. 
\end{align*}

We first establish the following lemma, which immediately implies part (a) of the theorem statement. 
\begin{lemma}\label{lem:dualproperties}
For all $t \le T$, $y^{(t)}$ is feasible for the dual SDP~\eqref{eq:dual}, and $\iprod{M,X^{(t)}}=\sum_{i} y^{(t)}_i$. 
\end{lemma}
\begin{proof}
We first check feasibility of the dual solution. First note that in every iteration $t \in [T]$, $\alpha^{(t)} \ge 0$ and $\lambda^{(t)} \ge 0$; this is because $M \succeq 0$, and hence $\diag(\alpha)^{-1/2} M \diag(\alpha)^{-1/2} \succeq 0$.  \anote{Is the above fact still true when $M$ is not PSD? Existence of a non-negative eigen value. This seems to be the only place where it fails for QP. Maybe other fix?} Hence $y^{(t)} \ge 0$. Moreover, by definition of $\lambda^{(t)}$
\begin{align*}
     M &\preceq \lambda^{(\ell)} \cdot \diag(\alpha^{(\ell)}) ~~\forall \ell \le T, ~~(\text{ since } \diag(\alpha^{(t)})^{-1/2} M \diag(\alpha^{(t)})^{-1/2} \preceq \lambda^{(t)} I) ,\\
    M&\preceq \frac{1}{t} \sum_{\ell=1}^t \lambda^{(\ell)} \cdot \diag(\alpha^{(\ell)}) = \frac{1}{t} \sum_{\ell=1}^t \diag(y^{(\ell)}).     
\end{align*}

Finally, we establish $\iprod{M,X^{(t)}}=\sum_{i} y^{(t)}_i$. Note that by definition $v^{(\ell)}= \sqrt{n} \diag(\alpha^{(\ell)}) u^{(\ell)}$, where $u^{(\ell)}$ is the top eigenvector of $(\diag(\alpha)^{-1/2} M \diag(\alpha)^{-1/2})$, and $\lambda^{(\ell)}$ is its eigenvalue. Hence
\begin{align*}
    \iprod{M,X^{(t)}} &= \frac{1}{t} \sum_{\ell=1}^t \iprod{ M, v^{(\ell)} (v^{(\ell)})^{\top} }= \frac{1}{t} \sum_{\ell=1}^t (v^{(\ell)})^{\top} M v^{(\ell)} \\
    &= n \frac{1}{t} \sum_{\ell=1}^t \Big((u^{(\ell)})^{\top} \diag(\alpha^{(\ell)})^{1/2} M \diag(\alpha^{(\ell)} u^{(\ell)}\Big) =  \frac{1}{t} \sum_{\ell=1}^t \lambda^{(\ell)} \cdot n\\
    \text{On the other hand, }~ \sum_{i=1}^n y^{(t)}_i &= 
    \sum_{i=1}^n \frac{1}{t} \sum_{\ell=1}^t \lambda^{(\ell)} \alpha^{(\ell)}(i) = \frac{1}{t} \sum_{\ell=1}^t \lambda^{(\ell)} \cdot \sum_{i=1}^n \alpha^{(\ell)}(i) =  \frac{1}{t} \sum_{\ell=1}^t \lambda^{(\ell)} \cdot n.
\end{align*}
This proves the lemma. 
\end{proof}

We now complete the proof of Theorem~\ref{thm:sdp-guarantee}. 
\begin{proof}
Recall that $\widehat{X}=X^{(T)}, \widehat{y}=y^{(T)}$.  Consider the SDP solution $X' = \tfrac{1}{1+\eps} \widehat{X}$. From Lemma~\ref{lem:dualproperties}, we see that $y^{(T)}$ is feasible and 
\begin{align*}
    \iprod{M,X'}&= \frac{1}{1+\eps} \iprod{M, \widehat{X}} =  \frac{1}{1+\eps} \sum_{i=1}^n \widehat{y}(i) \ge \frac{1}{1+\eps}\cdot \text{sdpval},
\end{align*}
where the last inequality follows from weak duality of the SDP. Hence it suffices to show that $X'$ is feasible i.e., $\widehat{X}_{ii} \le 1+\eps$ for all $i \in [n]$.  

We prove $\max_{i \in [n]} \widehat{X}_{ii} \le 1+\eps$ by following the same multiplicative weight analysis in \cite{Kalethesis} (see Section 2, Theorem 5), but only restricted to the $n$ constraints of the form $X_{ii} \le 1$.
We sketch the argument here. There is one expert for each $i \in [n]$ corresponding to the constraint $X_{ii} \le 1$. At each iteration $t$, we consider a probability distribution $p^{(t)}=\tfrac{1}{n} \alpha^{(t)}$. The loss of expert $i$ at time $t$ is given by $m^{(t)}(i)=\tfrac{1}{n}((v^{(t)}_i)^2-1)$. It is easy to see that 
\anote{why is $X_{ii} \le n$? Needed for width bound.}


\end{proof}


